US Salary History Bans -- Strategic Disclosure by Job Applicants and the Gender Pay Gap

I study the effects of US salary history bans which restrict employers from inquiring about job applicants' pay history during the hiring process, but allow candidates to voluntarily share information. Using a difference-in-differences design, I show that these policies narrowed the gender pay gap significantly by 2 p.p., driven almost entirely by an increase in female earnings. The bans were also successful in weakening the auto-correlation between current and future earnings, especially among job-changers. I provide novel evidence showing that when employers could no longer nudge candidates for information, the likelihood of voluntarily disclosing salary history decreased among job applicants and by 2 p.p. more among women. I then develop a salary negotiation model with asymmetric information, where I allow job applicants to choose whether to reveal pay history, and use this framework to explain my empirical findings on disclosure behavior and gender pay gap.

==> Proofs_of_Propositions <==
%#####################################################################
%#####################################################################
\section{Proofs of Propositions \label{ProofsOfPropositions}}
\renewcommand{\thefigure}{E\arabic{figure}}
\renewcommand{\thetable}{E\arabic{table}}
\renewcommand{\theequation}{E\arabic{equation}} 
\setcounter{figure}{0}
\setcounter{table}{0}
\setcounter{equation}{0}


\begin{proposition}{1}{}\label{propalt:existnondisc}
Given $(z,c,z',e,c_{e1},c_{e0},w_{L},w_{H})$ $\exists\  \tilde{f}_{e}\in\left(0,1\right)$ such that:
\begin{itemize}
    \item[1.] $\forall\  f_{L}>\tilde{f}_{e}$ there is a \textbf{Separating Equilibrium} where the firm commits to offering $\hat{w}_{e1}$ to high-earners if they disclose, and $\tilde{w}_{e0}$ to everyone else regardless of their disclosure. 
    Low-earners (i.e., $w=w_{L}$) optimally choose to not disclose ($d=0$) and high-earners (i.e., $w=w_{H}$) choose to disclose ($d=1$).  
    \item[2.] $\forall\  f_{L}\leq\tilde{f}_{e}$ there is a \textbf{Pooling Equilibrium} where the firm offers a flat wage $\hat{w}_{e0}$ regardless of disclosure $d$ and initial wage $w$ (if disclosed).
    Both high and low-earners optimally choose to not disclose ($d=0$).  
    \item[3.] $\tilde{f}_{1}<\tilde{f}_{0}$. 
\end{itemize}
\end{proposition} 

\begin{flushleft}\textbf{Proof:}\end{flushleft} 
I prove this proposition by first characterizing the optimal wage offers under which workers find it optimal to not deviate from equilibrium strategies and then show why these wage offers are optimal for the firm. 
Given $(z,c,z',c_{e1}^{'},c_{e0}^{'},w_{L},w_{H},u(.))$ I first define four threshold wages $(\hat{w}_{e1},\hat{w}_{e0},\tilde{w}_{e1},\tilde{w}_{e0})$ that satisfy the following equations\footnote{I show later what happens when one or more of these threshold wage values do not exist.}:
\begin{align}
u(\hat{w}_{e1}, z')-c_{e1} &= u(w_{H},z)- c \label{eq:highdisc} \\
u(\hat{w}_{e0}, z')-c_{e0} &= u(w_{H},z)- c \label{eq:highnodisc} \\
u(\tilde{w}_{e1}, z')-c_{e1} &= u(w_{L},z)- c \label{eq:lowdisc} \\
u(\tilde{w}_{e0}, z')-c_{e0} &= u(w_{L},z)- c \label{eq:lownodisc} 
\end{align}
$\because\  c_{e1}>c_{e0}$, (\ref{eq:highdisc}) and (\ref{eq:highnodisc}) $\Rightarrow\  \hat{w}_{e1}>\hat{w}_{e0}$. 
Similarly, I can show that $\tilde{w}_{e1}>\tilde{w}_{e0}$ using (\ref{eq:lowdisc}) and (\ref{eq:lownodisc}). 
Again, $\because\  w_{H}>w_{L}$, using (\ref{eq:highdisc}), (\ref{eq:lowdisc}), and Assumption \ref{Assumputil} I can argue that $\hat{w}_{e1}>\tilde{w}_{e1}$.
Following similar logic, I can show $\hat{w}_{e0}>\tilde{w}_{e0}$. 

Therefore, in a separating equilibrium, for any worker with $w=w_{H}$:
\begin{align}
& u(\hat{w}_{e1}, z')-c_{e1} > u(w_{L},z)-c & \  (\text{using }\ref{eq:highdisc}\text{ and }\text{Assumption}\  \ref{Assumputil}) &\nonumber \\
\Rightarrow\  & u(\hat{w}_{e1}, z')-c_{e1} > u(\tilde{w}_{e0}, z')-c_{e0} &\  (\text{using }\ref{eq:lownodisc}) \nonumber \\
\Rightarrow\  & \mathbf{d}(w=w_{H}, \text{Separating}) = 1\  \qedsymbol \nonumber 
\end{align}
Again, in a separating equilibrium for a worker with $w=w_{L}$:
\begin{align}
& u(\tilde{w}_{e0}, z')-c_{e0} < u(\tilde{w}_{e0}, z')-c_{e1} & (\text{using Assumption }\ref{Assumpprivacycost}) \nonumber \\
\Rightarrow\  & \mathbf{d}(w=w_{L}, \text{Separating}) = 0\  \qedsymbol \nonumber 
\end{align}
In a pooling equilibrium for any worker:
\begin{align}
& u(\hat{w}_{e0}, z')-c_{e0} > u(\hat{w}_{e0}, z')-c_{e1} & (\text{using Assumption }\ref{Assumpprivacycost}) \nonumber \\
\Rightarrow\  & \mathbf{d}(w, \text{Pooling}) = 0\  \forall\  w\in\left\{w_{L},w_{H}\right\}\  \qedsymbol \nonumber 
\end{align}
Therefore, in both separating and pooling equilibria, given the new firm's optimal wage offers, both types of workers have no incentive to deviate from the equilibria strategies above. 
Next, I verify that the the wage offers that the new firm commits to result in the maximum expected profit for the firm. 


First, I show why there can be only the two types of equilibria above: a separating equilibria where high-earners disclose but low-earners do not disclose, and a pooling equilibria where no types of workers disclose. 
To see this, let's consider the case where both types of workers disclose. In order to incentivize them to disclose while still accepting the new job, the firm has to offer $\hat{w}_{e1}$ to the high-earner and $\tilde{w}_{e1}$ to the low-earner. 
However, once high-earners disclose the firm can identify low-earners and therefore instead of offering them $\tilde{w}_{e1}$ they can be offered a lower wage $\tilde{w}_{e0}$ while incentivizing them to not disclose. 
Therefore, incentivizing both types of workers to disclose is not optimal for the new firm. 
Similarly, let's consider the case where the high-earners do not disclose and the low-earners disclose. 
In order to incentivize them to follow these disclosure decisions in equilibrium and still accept the new job, the new firm has to offer the high-earner $\hat{w}_{e0}$ and the low-earner $\tilde{w}_{e1}$. 
Both high and low-earners would be receiving just their outside option surplus at these offered wages. 
Then the low-earner has an incentive to not disclose and earn $\hat{w}_{e0}$ which will give them a utility value of ($u(w_{H},z)-c$) which is greater than their outside option. 
Again, there cannot be an equilibrium where the high-earner does not disclose and the low-earner discloses. 


Second, I show why it's optimal for the firm to offer the separating and pooling wages as above. 
Consider the separating equilibria where high-earners disclose and low-earners do not disclose. 
In order to incentivize high-earners to disclose while still accepting the new offer, they have to be paid at least $\hat{w}_{e1}$ which gives them just enough utility to match their outside option. 
Similarly, in order to incentivize low-earners to accept the offer while not disclosing, they need to be paid a wage slightly higher than $\tilde{w}_{e0}$. 
Any wages higher than these offers would imply less expected profits for the firm, while any wages lower than these values would incentivize workers to not accept the offer and leave the firm with 0 output. 
Now consider the pooling equilibria where the firm offers both workers $\hat{w}_{e0}$, by which the firm extracts full surplus from the high-earner and provides some rent to the low-earner. 
For any wages higher than this offer, the firm would lose out on profits. 
For any wage between $\tilde{w}_{e0}$ and $\hat{w}_{e0}$, the high-earners would not accept the offer, the low-earners would still accept the offer and the firm would lose out on expected profits. 
For any wage less than $\tilde{w}_{e0}$, even low-earners would no longer accept the offer and the firm would generate 0 output. 

Finally, I show when it's optimal for the firm to offer separating versus pooling wages as $f_{L}$ varies. 
Define the threshold value $\tilde{f}_{e}$ as follows:
\begin{equation}\label{eq:cutofffrac}\tilde{f}_{e} = \frac{\hat{w}_{e1}-\hat{w}_{e0}}{\hat{w}_{e1}-\tilde{w}_{e0}}\in(0,1),\  (\text{using }\ref{eq:highnodisc},\ref{eq:lownodisc}\text{ and Assumption }\ref{Assumputil})\end{equation}
Therefore, $\forall\  f_{L}>\tilde{f}_{e}$: 
\begin{align}
& f_{L} > \frac{\hat{w}_{e1}-\hat{w}_{e0}}{\hat{w}_{e1}-\tilde{w}_{e0}} \nonumber \\
\Rightarrow\  & f_{L}(\hat{w}_{e1}-\tilde{w}_{e0}) > \hat{w}_{e1}-\hat{w}_{e0} \nonumber \\
\Rightarrow\  & (1-f_{L})\hat{w}_{e1}+f_{L}\tilde{w}_{e0} < \hat{w}_{e0} \nonumber \\
\Rightarrow\  & z'-\Big[(1-f_{L})\hat{w}_{e1}+f_{L}\tilde{w}_{e0}\Big] > z' - \hat{w}_{e0} \nonumber \\
\Rightarrow\  & \text{Offer Separating Wages} \nonumber 
\end{align} 
Similarly, it can be proved that $\forall\  f_{L}\leq\tilde{f}_{e}$ it is optimal for the new firm to offer pooling wages. 

The third part of this proposition can be proved as follows.
\begingroup
\allowdisplaybreaks
\begin{align}
& u(x,z')-c' = u(w,z)-c \nonumber \\
\Rightarrow\  & \frac{\partial u}{\partial x}\frac{\partial x}{\partial c'} - 1 = 0 \nonumber \\
\Rightarrow\  & \frac{\partial x}{\partial c'} = -(\frac{\partial u}{\partial x})^{-1} \nonumber \\
\Rightarrow\  & \frac{{\partial}^{2}x}{\partial c'\partial w} = -\underbrace{(\frac{\partial u}{\partial x})^{-2}}_{>0}\underbrace{\frac{\partial^{2}u}{\partial x^{2}}}_{<0}\underbrace{\frac{\partial x}{\partial w}}_{>0}\  (\text{using Assumption }\ref{Assumputil}) \nonumber \\
\Rightarrow\  & \frac{{\partial}^{2}x}{\partial c'\partial w} > 0 \nonumber \\ 
\Rightarrow\  & \hat{w}_{10}-\tilde{w}_{10} > \hat{w}_{00}-\tilde{w}_{00} \nonumber \\
\Rightarrow\ & \frac{\hat{w}_{10}-\tilde{w}_{10}}{\hat{w}_{11}-\tilde{w}_{10}} > \frac{\hat{w}_{00}-\tilde{w}_{00}}{\hat{w}_{11}-\tilde{w}_{00}},\  (\text{using Assumptions }\ref{Assumpequalgender}\text{ and }\ref{Assumpnonconformity},\text{ and }\ref{eq:lownodisc}) \nonumber \\ 
\Rightarrow\  & \frac{\hat{w}_{10}-\tilde{w}_{10}}{\hat{w}_{11}-\tilde{w}_{10}} > \frac{\hat{w}_{00}-\tilde{w}_{00}}{\hat{w}_{01}-\tilde{w}_{00}} \nonumber \\ 
\Rightarrow\  & \frac{\hat{w}_{11}-\tilde{w}_{10}}{\hat{w}_{11}-\tilde{w}_{10}} < \frac{\hat{w}_{01}-\tilde{w}_{00}}{\hat{w}_{01}-\tilde{w}_{00}} \nonumber \\
\Rightarrow\  & \tilde{f}_{1} < \tilde{f}_{0}\  \qedsymbol\nonumber
\end{align}
\endgroup

\medskip

\begin{proposition}{2}{}\label{propalt:SHBchangedisc}
Given $(z,c,z',e,c_{11}=c_{01}>c_{00},w_{L},w_{H})$ $\exists\  \bar{c},\tilde{f}_{1},\tilde{f}_{0}$ such that\\
\textbf{Case A: }$\forall\  c_{10}\in(c_{00},\bar{c}),\  \forall\  f_{L}\in(\tilde{f}_{1},\tilde{f}_{0})$:
\begin{itemize}
    \item[1.] The new firm offers separating wages when $e=1$ and pooling wages when $e=0$. 
    \item[2.] $\text{Pr}(d=1|e=1)>\text{Pr}(d=1|e=0)$. 
    \item[3.] $\mathbb{E}(w^{'}|e=1, w=w_{H})>\mathbb{E}(w^{'}|e=0, w=w_{H})$. 
    \item[4.] $\mathbb{E}(w^{'}|e=1, w=w_{L})<\mathbb{E}(w^{'}|e=0, w=w_{L})$
\end{itemize}
\textbf{Case B: }$\forall\  c_{10}\in(c_{00},\bar{c}),\  \forall\  f_{L}\leq\tilde{f}_{1}$:
\begin{itemize}
    \item[1.] The new firm offers pooling wages both when $e=1$ and $e=0$. 
    \item[2.] $\text{Pr}(d=1|e=1)=\text{Pr}(d=1|e=0)=0$. 
    \item[3.] $\mathbb{E}(w^{'}|e=1, w=w_{H})>\mathbb{E}(w^{'}|e=0, w=w_{H})$. 
    \item[4.] $\mathbb{E}(w^{'}|e=1, w=w_{L})>\mathbb{E}(w^{'}|e=0, w=w_{L})$
\end{itemize}
\textbf{Case C: }$\forall\  c_{10}\in(c_{00},\bar{c}),\  \forall\  f_{L}\geq\tilde{f}_{0}$:
\begin{itemize}
    \item[1.] The new firm offers separating wages both when $e=1$ and $e=0$. 
    \item[2.] $\text{Pr}(d=1|e=1)=\text{Pr}(d=1|e=0)=(1-f_{L})$. 
    \item[3.] $\mathbb{E}(w^{'}|e=1, w=w_{H})>\mathbb{E}(w^{'}|e=0, w=w_{H})$. 
    \item[4.] $\mathbb{E}(w^{'}|e=1, w=w_{L})>\mathbb{E}(w^{'}|e=0, w=w_{L})$
\end{itemize}
\textbf{Case D: }$\forall\  c_{10}\geq\bar{c},\  \forall\  f_{L}\in(\tilde{f}_{1},\tilde{f}_{0})$:
\begin{itemize}
    \item[1.] The new firm offers separating wages when $e=1$ and pooling wages when $e=0$. 
    \item[2.] $\text{Pr}(d=1|e=1)>\text{Pr}(d=1|e=0)$. 
    \item[3.] $\mathbb{E}(w^{'}|e=1, w=w_{H})>\mathbb{E}(w^{'}|e=0, w=w_{H})$. 
    \item[4.] $\mathbb{E}(w^{'}|e=1, w=w_{L})\geq\mathbb{E}(w^{'}|e=0, w=w_{L})$
\end{itemize}
\textbf{Case E: }$\forall\  c_{10}\geq\bar{c},\  \forall\  f_{L}\leq\tilde{f}_{1}$:
\begin{itemize}
    \item[1.] The new firm offers pooling wages both when $e=1$ and $e=0$. 
    \item[2.] $\text{Pr}(d=1|e=1)=\text{Pr}(d=1|e=0)=0$. 
    \item[3.] $\mathbb{E}(w^{'}|e=1, w=w_{H})>\mathbb{E}(w^{'}|e=0, w=w_{H})$. 
    \item[4.] $\mathbb{E}(w^{'}|e=1, w=w_{L})>\mathbb{E}(w^{'}|e=0, w=w_{L})$
\end{itemize}
\textbf{Case F: }$\forall\  c_{10}\geq\bar{c},\  \forall\  f_{L}\geq\tilde{f}_{0}$:
\begin{itemize}
    \item[1.] The new firm offers separating wages both when $e=1$ and $e=0$. 
    \item[2.] $\text{Pr}(d=1|e=1)=\text{Pr}(d=1|e=0)=(1-f_{L})$. 
    \item[3.] $\mathbb{E}(w^{'}|e=1, w=w_{H})>\mathbb{E}(w^{'}|e=0, w=w_{H})$. 
    \item[4.] $\mathbb{E}(w^{'}|e=1, w=w_{L})>\mathbb{E}(w^{'}|e=0, w=w_{L})$
\end{itemize}
\end{proposition} 

\begin{flushleft}\textbf{Proof:}\end{flushleft}
First let's prove the results on disclosure rates. \\
Following Proposition \ref{propalt:existnondisc} I can see that $\forall\  f_{L}>\tilde{f}_{1}$ the new firm offers separating wages $(\hat{w}_{11},\tilde{w}_{10})$ when workers are asked $(e=1)$ and the firm offers pooling wages $(\hat{w}_{00})$ when workers are not asked $(e=0)$. 
Since high-earners disclose when separating wages are offered I have $\text{Pr}(d=1|e=1)=(1-f_{L})>0=\text{Pr}(d=0|e=0)\  \  \qedsymbol$. \\
Similarly, when $f_{L}<\tilde{f}_{1}\leq\tilde{f}_{0}$, the new firm offers pooling wages both when workers are asked and when not asked. 
Since both types of workers do not disclose in pooling equilibria, disclosure rates are zero, regardless of enquiry. 
Finally, when $f_{L}\geq\tilde{f}_{0}>\tilde{f}_{1}$, the firm offers separating wages both when workers are asked and when not asked. 
Since only high-earners disclose and the proportion of high-earners is fixed at $(1-f_{L})$, there are no differences in disclosure rates between the two cases. 


Next, I show the effects on wage offers for high-earners.
For Cases A and D, high-earners are offered $\hat{w}_{11}$ when asked and $\hat{w}_{00}$ when not asked. 
For Cases B and E, high-earners are offered $\hat{w}_{10}$ when asked and $\hat{w}_{00}$ when not asked. 
Finally, for Cases C and F, high-earners are offered $\hat{w}_{11}$ when asked and $\hat{w}_{01}$ when not asked. 
Using (\ref{eq:highdisc}), ($\ref{eq:highnodisc}$), and Assumptions \ref{Assumpprivacycost} and \ref{Assumpnonconformity} I can show $\hat{w}_{11}=\hat{w}_{01}>\hat{w}_{10}>\tilde{w}_{00}$. 
Therefore, $\mathbb{E}(w^{'}|e=1, w=w_{H})\geq\mathbb{E}(w^{'}|e=0, w=w_{H})\  \  \qedsymbol$.

Finally, I want to impose an upper bound on the value of $c_{10}$ which will ensure $\tilde{w}_{10}<\hat{w}_{00}$. 
This can be done as follows:
\begin{align}
& u(\tilde{w}_{00},z')-c_{00}=u(w_{L},z)-c < u(w_{H},z)-c = u(\hat{w}_{00},z')-c_{00} \nonumber \\
\Rightarrow\  & \tilde{w}_{00} < \hat{w}_{00} \label{Prop2eq01}
\end{align}
Furthermore,
\begin{align}
& u(x,z')-c' = u(w,z)-c \nonumber \\
\Rightarrow\  & \frac{\partial x}{\partial c'} = (\frac{\partial u}{\partial x})^{-1} > 0 \label{Prop2eq02}
\end{align}
The inequalities in (\ref{Prop2eq01}) and (\ref{Prop2eq02}) imply that $\exists\  \bar{c}$ such that $\forall\  c_{10}\in(c_{00},\bar{c})$ I have $\tilde{w}_{00}<\tilde{w}_{10}<\hat{w}_{00}$. 
And $\forall\  c_{10}\geq\bar{c}$ I have $\tilde{w}_{00}<\hat{w}_{00}\leq\tilde{w}_{10}$. \\
For Case A, low-earners are offered $\tilde{w}_{10}$ when asked and $\hat{w}_{00}$ when not asked. 
Therefore $\mathbb{E}(w^{'}|e=1, w=w_{L})<\mathbb{E}(w^{'}|e=0, w=w_{L})\  \  \qedsymbol$. \\
For Cases B and E, low-earners are offered $\hat{w}_{10}$ when asked and $\hat{w}_{00}\  (<\hat{w}_{10})$ when not asked. 
Therefore, $\mathbb{E}(w^{'}|e=1, w=w_{L})>\mathbb{E}(w^{'}|e=0, w=w_{L})\  \  \qedsymbol$. \\
For Cases C and F, low-earners are offered $\tilde{w}_{10}$ when asked and $\tilde{w}_{00}$ when not asked. 
Therefore, $\mathbb{E}(w^{'}|e=1, w=w_{L})>\mathbb{E}(w^{'}|e=0, w=w_{L})\  \  \qedsymbol$. \\
For Case D, low-earners are offered $\tilde{w}_{10}$ when asked and $\hat{w}_{00}$ when not asked. 
Therefore, $\mathbb{E}(w^{'}|e=1, w=w_{L})\geq\mathbb{E}(w^{'}|e=0, w=w_{L})\  \  \qedsymbol$.  


\medskip
\begin{proposition}{3}{}\label{propalt:diffgenderdist}
Given ($z,c,z',c_{11}=c_{01}>c_{10}^{M},c_{00},w_{L},w_{H}$) $\exists\  \underline{c}_{F}$ ($>c_{10}^{M}$) such that \\ 
$\forall\  c_{10}^{F}\in\left(c_{10}^{M},\underline{c}_{F}\right)$, $\exists\  \tilde{f}_{1M},\bar{f},\tilde{f}_{0F}$ such that $\forall\  f_{L}^{M}<\tilde{f}_{1M}<\bar{f}<f_{L}^{F}<\tilde{f}_{0F}$:
\begin{itemize}
    \item[1.] Firm offers separating wages to female workers and pooling wages to male workers when asked, and pooling wages to all workers when not asked. 
    \item[2.] $\text{Pr}(d=1|e=1,k=F)>\text{Pr}(d=1|e=1,k=M)$.
    \item[3.] $\text{Pr}(d=1|e=1)>\text{Pr}(d=1|e=0)=0$.
    \item[4.] $\mathbb{E}(w'|e=1,w=w_{L},k=F)<\mathbb{E}(w'|e=0,w=w_{L},k=F)$, \\ $\mathbb{E}(w'|e=1,w=w_{L},k=M)>\mathbb{E}(w'|e=0,w=w_{L},k=M)$. 
    \item[5.] $\mathbb{E}(w'|e=1,w=w_{H},k)>\mathbb{E}(w'|e=0,w=w_{H},k)\  \forall\  k\in\left\{F,M\right\}$.
    \item[6.] $\mathbb{E}(w'|e=0,k=F)-\mathbb{E}(w'|e=0,k=M)>\mathbb{E}(w'|e=1,k=F)-\mathbb{E}(w'|e=1,k=M)$.
\end{itemize}
\end{proposition}

\begin{flushleft}\textbf{Proof:}\end{flushleft}
First I prove the results on disclosure rates and wages for men. 
Given $(z,c,z',c_{11}=c_{01}>c_{10}^{M}>c_{00},w_{L},w_{H})$ define $\tilde{f}_{1M}$ following (\ref{eq:cutofffrac}) as:
\begin{equation}\tilde{f}_{1M} = \frac{\hat{w}_{11}-\hat{w}_{10}^{M}}{\hat{w}_{11}-\tilde{w}_{10}^{M}}\in(0,1)\nonumber\end{equation}
If $f_{L}^{M}<\tilde{f}_{1M}$ then by Proposition \ref{propalt:SHBchangedisc}, the firm would offer pooling wages to men both when they are asked and when they are not asked. 
Therefore, both when they are asked and when they're not, disclosure rates among men are zero. 
Regardless of whether $c_{10}^{M}$ is high, Cases B and E in Proposition \ref{propalt:SHBchangedisc} show that for both high and low-earning men, wage offers are lower when workers are not asked in comparison to when they're asked. 

Second, I prove the results on disclosure rates and wages for women. 
To do this, I argue that $\tilde{f}_{0F}\text{ and }\tilde{f}_{0M}$, which are the $\tilde{f}_{0}$ equivalent (from Proposition \ref{propalt:SHBchangedisc}) for women and men respectively, are equal. 
To see this, I use use (\ref{eq:cutofffrac}) as follows:
\begin{equation}\tilde{f}_{0F} = \frac{\hat{w}_{01}-\hat{w}_{00}}{\hat{w}_{01}-\tilde{w}_{00}}=\tilde{f}_{0M}\nonumber\end{equation}
Intuitively, since there are no differences in disclosure and non-disclosure costs between men and women when they are not asked, and so the proportion of low-earners below which the firm offers pooling wages ($\tilde{f}_{0F},\tilde{f}_{0M}$) are the same. 

Next, I argue that $\tilde{f}_{1M}\in(\tilde{f}_{1F},\tilde{f}_{0F}$ where $\tilde{f}_{1F}\text{ and }\tilde{f}_{1M}$ are the $\tilde{f}_{1}$ (from Proposition \ref{propalt:SHBchangedisc}) for women and men respectively. 
The first inequality $\tilde{f}_{1F}<\tilde{f}_{1M}$ can be proved using the single crossing property of $u(w,z)-c$ in the same way as the last result of Proposition \ref{propalt:existnondisc}. The second inequality (i.e., $\tilde{f}_{1M}<\tilde{f}_{0F}$ can also be proved in the same way by replacing $\tilde{f}_{0F}$ with $\tilde{f}_{0M}$. 
Therefore $f_{L}^{F}\in(\tilde{f}_{1M},\tilde{f}_{0F})\Rightarrow f_{L}^{F}\in(\tilde{f}_{1F},\tilde{f}_{0F})$ and so the new firm offers separating wages to female workers when they are asked and pooling wages when not asked (by Proposition \ref{propalt:SHBchangedisc}).
Since only high-earners disclose when separating wages are offered, the disclosure rate is $(1-f_{L}^{F})$ when women are asked and 0 when not asked. 
This shows that disclosure rates are higher among women than men on average, when workers are asked. 
It also shows that disclosure rates are higher on average when workers are asked than when not asked. 
Cases A and D in Proposition \ref{propalt:SHBchangedisc} show that for high earning women, wages decrease when workers are not asked. 
Finally, I prove the results on wages for low-earning women and use this for the result on gender wage gap.
Define $\bar{f}$ as follows:
\begin{equation}\label{frac:cutoffgwg}\bar{f} = \frac{\hat{w}_{11}-\hat{w}_{10}^{M}}{\hat{w}_{11}-\tilde{w}_{10}^{F}}\end{equation}
First, $c_{10}^{M}<c_{10}^{F}\Rightarrow\  \tilde{w}_{10}^{M}<\tilde{w}_{10}^{F}\Rightarrow\  \frac{\hat{w}_{11}-\hat{w}_{10}^{M}}{\hat{w}_{11}-\tilde{w}_{10}^{M}}<\frac{\hat{w}_{11}-\hat{w}_{10}^{M}}{\hat{w}_{11}-\tilde{w}_{10}^{F}}\Rightarrow\  \tilde{f}_{1M}<\bar{f}$. \\
Next, define $\bar{f}(x)$ as:
\begin{equation}\bar{f}(x) = \frac{\hat{w}_{11}-\hat{w}_{10}^{M}}{\hat{w}_{11}-x}\nonumber\end{equation}
Note that $\bar{f}(\tilde{w}_{10}^{M}) = \tilde{f}_{1M}$, $\bar{f}(\tilde{w}_{10}^{F})=\bar{f}$ and $\frac{\partial}{\partial x}\bar{f}(x)>0$. I also know that $\tilde{f}_{1M}<\tilde{f}_{0F}$ and $\frac{\partial}{\partial c_{10}^{F}}\tilde{w}_{10}^{F}>0$. Therefore $\exists\  \hat{c}_{F}>c_{10}^{M}$ such that $\bar{f}(\tilde{w}_{10}^{F})\in(\tilde{f}_{1M},\tilde{f}_{0F})$. 
Following Proposition \ref{propalt:SHBchangedisc} define $\bar{c}_{F}>c_{10}^{M}$ as the upper-bound on $c_{10}^{F}$ such that $\tilde{w}_{10}^{F}<\hat{w}_{00}$. 
Finally, define $\underline{c}_{F}:=\min(\bar{c}_{F},\hat{c}_{F})>c_{10}^{M}$. 

Then, by Case D of Proposition \ref{propalt:SHBchangedisc}, wage offers of low-earning women are higher when workers are not asked than when they're asked. Finally, 
\begin{align}
& f_{L}^{F} > \bar{f} \nonumber \\ 
\Rightarrow\  & f_{L}^{F} > \frac{\hat{w}_{11}-\hat{w}_{10}^{M}}{\hat{w}_{11}-\tilde{w}_{10}^{F}} \nonumber \\ 
\Rightarrow\  & f_{L}^{F}\tilde{w}_{10}^{F} + (1-f_{L}^{F})\hat{w}_{11} < \hat{w}_{10}^{M} \nonumber \\
\Rightarrow\  & \hat{w}_{00} - \Big[f_{L}^{F}\tilde{w}_{10}^{F} + (1-f_{L}^{F})\hat{w}_{11}\Big] > \hat{w}_{00} - \hat{w}_{10}^{M} \nonumber \\
\Rightarrow\  & \mathbb{E}(w'|e=0,k=F)-\mathbb{E}(w'|e=0,k=M)>\mathbb{E}(w'|e=1,k=F)-\mathbb{E}(w'|e=1,k=M)\  \qedsymbol \nonumber 
\end{align}

\subsection*{Non-Existence of Threshold Values \label{proofnonexistence}}

The existence of the threshold values $\tilde{f}_{ek},\bar{c}_{k},\underline{c}_{k}$ in the propositions above depend on the existence of the threshold values of wages $\tilde{w}_{ed}^{k},\hat{w}_{ed}^{k}$. 
In this section I show what happens when these threshold wage values do not exist. To recap, the four threshold wages for each enquiry status are as follows:
\begin{align}
u(\hat{w}_{e1}, z')-c_{e1} &= u(w_{H},z)- c \nonumber \\
u(\hat{w}_{e0}, z')-c_{e0} &= u(w_{H},z)- c \nonumber \\
u(\tilde{w}_{e1}, z')-c_{e1} &= u(w_{L},z)- c \nonumber \\
u(\tilde{w}_{e0}, z')-c_{e0} &= u(w_{L},z)- c \nonumber 
\end{align}

Since the firm is risk neutral it has no incentive to offer wages higher than $z'$. 
The following can be proved:
\begin{align}
\exists\  \hat{w}_{e1}\Rightarrow\  \exists\  \hat{w}_{e0}\Rightarrow\  \exists\  \tilde{w}_{e0} \label{threshexist01}
\end{align}
Intuitively, the cost of disclosing information $c_{e1}$ is higher than the cost of not disclosing information $c_{e0}$ and high-earners have to be compensated more than low-earners. 
Therefore, if the firm can offer a wage to incentivize high-earners to accept the offer while disclosing their wages, they can also incentivize both high and low-earners when they do not disclose information. 
This is true both when workers are asked and when they are not asked. 
\begin{comment}
In a similar way, the following can be proved:
\begin{align}
\exists\  (\hat{w}_{11}=\hat{w}_{01})\Rightarrow\  \exists\  \hat{w}_{10}^{F}\Rightarrow\  \exists\  \hat{w}_{10}^{M}\Rightarrow\  \exists\  \hat{w}_{00}\Rightarrow\  \exists\  \tilde{w}_{10}^{F}\Rightarrow\  \exists\  \tilde{w}_{10}^{M}\Rightarrow\  \exists\  \tilde{w}_{00}\label{threshexist02}
\end{align}
\end{comment}

Therefore, if $\nexists\  \tilde{w}_{e0}$ implies the new firm would not be able to offer wages that would incentivize even low-earners to accept the offer and therefore there will be no turnover. \\
If $\nexists\  \hat{w}_{10}$ implies that the new firm would not be able to compensate high earners and only low-earners would accept the offer. 
Since it costs the firm to incentivize workers to disclose the firm would offer low-earners $\tilde{w}_{e0}$. \\
Finally, if $\nexists\  \hat{w}_{11}$ then again the firm would offer the pooling wage $\hat{w}_{10}$ to all workers since it cannot compensate high-earners for disclosing information. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> SalaryHistoryBanBiblio.tex <==
@article{AganStarr2017,
   author = {Agan, Amanda and Starr, Sonja},
   title = {Ban the Box, Criminal Records, and Racial Discrimination: A Field Experiment*},
   journal = {The Quarterly Journal of Economics},
   volume = {133},
   number = {1},
   pages = {191-235},
   year = {2017},
   type = {Journal Article}
}

@article{Akerlof1970,
    author = {Akerlof, George A.}, 
    title = {The Market for ``Lemons": Quality Uncertainty and the Market Mechanism},
    journal = {The Quarterly Journal of Economics}, 
    volume = {84}, 
    number = {3},
    year = {1970},
    pages = {488-500}, 
    type = {Journal Article}
}

@article{AganCowgillGee2020b,
	author = {Agan, Amanda and Cowgill, Bo and Gee, Laura},
	title = {Do Workers Comply with Salary History Bans? A Survey on Voluntary Disclosure, Adverse Selection and Unravelling}, 
	journal = {AEA Papers and Proceedings, Forthcoming},
	volume = {110},
	year = {2020},
	type = {Journal Article}
}

@article{AganCowgillGee2020a,
	author = {Agan, Amanda and Cowgill, Bo and Gee, Laura},
	title = {Salary Disclosure and Hiring: Field Experimental Evidence from a Two-Sided Audit Study},
	journal = {Working Paper},
	year = {2020},
	type = {Journal Article}
}

@article{AgrawalLaceteraLyons2013,
   author = {Agrawal, Ajay K. and Lacetera, Nicola and Lyons, Elizabeth},
   title = {Does Information help or hinder job applicants from less developed countries in online markets?},
   journal = {NBER Working Paper No. 18720},
   year = {2013},
   type = {Journal Article}
}

@article{AltonjiPierret2001,
   author = {Altonji, Joseph G. and Pierret, Charles R.},
   title = {Employer Learning and Statistical Discrimination*},
   journal = {The Quarterly Journal of Economics},
   volume = {116},
   number = {1},
   pages = {313-350},
   year = {2001},
   type = {Journal Article}
}

@article{AmanatullahMorris2010,
   author = {Amanatullah, Emily T. and Morris, Michael W.},
   title = {Negotiating Gender Roles: Gender Differences in Assertive Negotiating are Mediated by Women's Fear of Backlash and Attenuated When Bargaining When Negotiating on Behalf of Others},
   journal = {Journal of Personality and Social Psychology},
   volume = {98},
   number = {2},
   pages = {256-267},
   year = {2010},
   type = {Journal Article}
}

@article{AmanatullahTinsley2013,
   author = {Amanatullah, Emily T. and Tinsley, Catherine H.},
   title = {Punishing female negotiators for asserting too much or not enough: Exploring why advocacy moderates backlash against assertive female negotiators},
   journal = {Organizational Behavior and Human Decision Processes},
   volume = {120},
   number = {1},
   pages = {110-122},
   year = {2013},
   type = {Journal Article}
}

@article{AutorScarborough2008,
   author = {Autor, David H. and Scarborough, David},
   title = {Does Job Testing Harm Minority Workers? Evidence from Retail Establishments*},
   journal = {The Quarterly Journal of Economics},
   volume = {123},
   number = {1},
   pages = {219-277},
   year = {2008},
   type = {Journal Article}
}

@book{BabcockLaschever2004,
   author = {Babcock, Linda and Laschever, Sara},
   title = {Women Don't Ask: Negotiation and The Gender Divide},
   publisher = {Princeton University Press},
   year = {2004},
   type = {Book}
}

@article{Bakeretal2019,
   author = {Baker, Michael and Halberstam, Yosh and Kroft, Kory and Mas, Alexandre and Messacar, Derek},
   title = {Pay Transparency and The Gender Pay Gap},
   journal = {NBER Working Paper No. 25834},
   year = {2019},
   type = {Journal Article}
}

@article{BarachHorton2020,
   author = {Barach, Moshe and Horton, John, J.},
   title = {How do employers use compensation history? Evidence from a Field Experiment},
   journal = {Journal of Labor Economics},
   volume = {39}, 
   number = {1}, 
   pages = {193-218},
   year = {2020},
   type = {Journal Article}
}


@article{BartikNelson2016,
   author = {Bartik, A.W. and Nelson, S.T.},
   title = {Credit Reports as Resumes: The Incidence of pre-employment credit screening},
   journal = {MIT Economics Working Paper No 16-01},
   year = {2016},
   type = {Journal Article}
}

@article{CullenPerezTruglia2021,
    author = {Cullen, Zoe and Perez-Truglia, Ricardo},
    title = {How Much Does Your Boss Make? The Effects of Salary Comparisons}, 
    journal = {Journal of Political Economy}, 
    year = {2021}, 
    type = {Journal Article}
}

@article{Bennedsenetal2019,
   author = {Bennedsen, Morten and Simintzi, Elena and Tsoutsoura, Margarita and Wolfenzon, Daniel},
   title = {Do Firms Respond to Gender Pay Gap Transarency?},
   journal = {NBER Working Paper No. 25435},
   year = {2019},
   type = {Journal Article}
}

@article{BertrandGoldinKatz2010,
   author = {Bertrand, Marianne and Goldin, Claudia and Katz, Lawrence F.},
   title = {Dynamics of the Gender Gap for Young Professionals in the Financial and Corporate Sectors},
   journal = {American Economic Journal: Applied Economics},
   volume = {2},
   number = {3},
   pages = {228-55},
   year = {2010},
   type = {Journal Article}
}

@article{BlackabyBoothFrank2005,
   author = {Blackaby, David and Booth, Alison L and Frank, Jeff},
   title = {Outside Offers and the Gender Pay Gap: Empirical Evidence from the UK Academic Labour Market},
   journal = {The Economic Journal},
   volume = {115},
   number = {501},
   pages = {F81-F107},
   year = {2005},
   type = {Journal Article}
}

@article{BlauKahn2017,
   author = {Blau, Francine D. and Kahn, Lawrence M.},
   title = {The Gender Wage Gap: Extent, Trends, and Explanations},
   journal = {Journal of Economic Literature},
   volume = {55},
   number = {3},
   pages = {789-865},
   year = {2017},
   type = {Journal Article}
}

@article{Blundelletal2004,
	author = {Blundell, R. and Costa-Dias, Monica and Meghir, Costas and Van-Reenen, John},
	title = {Evaluating the Employment Impact of a Mandatory Job Search Program},
	journal = {Journal of European Economic Association},
	volume = {2},
	number = {4},
	pages = {569-606},
	year = {2004},
	type = {Journal Article}
}

@article{BowlesBabcockLai2007,
   author = {Bowles, Hannah Riley and Babcock, Linda and Lai, Lei},
   title = {Social incentives for gender differences in the propensity to initiate negotiations: Sometimes it does hurt to ask},
   journal = {Organizational Behavior and Human Decision Processes},
   volume = {103},
   number = {1},
   pages = {84-103},
   year = {2007},
   type = {Journal Article}
}

@article{Burksetal2015,
   author = {Burks, Stephen V. and Cowgill, Bo and Hoffman, Mitchell and Housman, Michael},
   title = {The Value of Hiring through Employee Referrals *},
   journal = {The Quarterly Journal of Economics},
   volume = {130},
   number = {2},
   pages = {805-839},
   year = {2015},
   type = {Journal Article}
}

@article{CliffordShoag2016,
   author = {Clifford, Robert and Shoag, Daniel},
   title = {"No More Credit Score": The Effect of Employer Credit Check Bans on Employment},
   journal = {HKS Policy Briefs},
   year = {2016},
   type = {Journal Article}
}

@article{Deardenetal2001,
	author = {Dearden, L. and Emmerson, C. and Frayne, C. and Goodman, A. and Ichimura, H. and Meghir, C.},
	title = {Education Maintenance Allowance: The First Year A Quantitative Evaluation},
	journal = {Department for Education and Employment, Research Report No. 257},
	year = {2001},
	type = {Journal Article}
}

@article{Deardenetal2002,
	author = {Dearden, L. and Emmerson, C. and Frayne, C. and Meghir, C.},
	title = {Education Maintenance Allowance: The First Two Years A Quantitative Evaluation},
	journal = {Department for Education and Skills, Research Report No. 352},
	year = {2002},
	type = {Journal Article}
}

@article{DevaroWaldman2012,
   author = {DeVaro, Jed and Waldman, Michael},
   title = {The Signaling Role of Promotions: Further Theory and Empirical Evidence},
   journal = {Journal of Labor Economics},
   volume = {30},
   number = {1},
   pages = {91-147},
   year = {2012},
   type = {Journal Article}
}

@article{Dittrichetal2014,
   author = {Dittrich, Marcus and Knabe, Andreas and Leipold, Kristina},
   title = {Gender Differences in Experimental Wage Negotiations},
   journal = {Economic Inquiry},
   volume = {52},
   number = {2},
   pages = {862-873},
   year = {2014},
   type = {Journal Article}
}

@article{DoleacHansen2017,
   author = {Doleac, Jennifer L. and Hansen, Benjamin},
   title = {Moving to Job Opportunities? The Effect of "Ban the Box" on the Composition of Cities},
   journal = {American Economic Review},
   volume = {107},
   number = {5},
   pages = {556-59},
   year = {2017},
   type = {Journal Article}
}

@article{DoleacHansen2018,
   author = {Doleac, Jennifer L. and Hansen, Benjamin},
   title = {The Unintended Consequences of Ban the Box: Statistical Discrimination and Employment Outcomes When Criminal Histories are Hidden},
   year = {2018},
   type = {Journal Article}
}

@article{Eeckhout2006,
   author = {Eeckhout, Jan},
   title = {Employer Learning and General Human Capital},
   journal = {Working Paper},
   year = {2006},
   type = {Journal Article}
}

@article{Eurofound2018,
   author = {Eurofound},
   title = {Pay Transparency in Europe: First Experiences with Gender Pay Audits and Reports in Four Member States},
   journal = {Publications Office of the European Union, Luxemborg},
   year = {2018},
   type = {Journal Article}
}

@article{Exleyetal2018,
   author = {Exley, Christine L. and Niederle, Muriel and Vesterlund, Lise},
   title = {Knowing When to Ask: The Cost of Leaning In},
   journal = {Working Paper},
   year = {2018},
   type = {Journal Article}
}

@article{Farberetal2015,
   author = {Farber, Henry S. and Silverman, Dan and Wachter, Till von},
   title = {Factors Determining Callbacks to Job Applicants by the Unemployed: An Audit Study},
   journal = {NBER Working Paper No. 21689},
   year = {2015},
   type = {Journal Article}
}

@article{Goldin2014,
   author = {Goldin, Claudia},
   title = {A Grand Gender Convergence: Its Last Chapter},
   journal = {American Economic Review},
   volume = {104},
   number = {4},
   pages = {1091-1119},
   year = {2014},
   type = {Journal Article}
}

@article{Goldinetal2017,
   author = {Goldin, Claudia and Kerr, Sari Pekkala and Olivetti, Claudia and Barth, Erling},
   title = {The Expanding Gender Earnings Gap: Evidence from the LEHD-2000 Census},
   journal = {American Economic Review},
   volume = {107},
   number = {5},
   pages = {110-14},
   year = {2017},
   type = {Journal Article}
}

@article{GoldinRouse2000,
   author = {Goldin, Claudia and Rouse, Cecilia},
   title = {Orchestrating Impartiality: The Impact of "Blind" Auditions on Female Musicians},
   journal = {American Economic Review},
   volume = {90},
   number = {4},
   pages = {715-741},
   year = {2000},
   type = {Journal Article}
}

@article{HallKrueger2012,
   author = {Hall, Robert E. and Krueger, Alan B.},
   title = {Evidence on the Incidence of Wage Posting, Wage Bargaining, and On-the-Job Search},
   journal = {American Economic Journal: Macroeconomics},
   volume = {4},
   number = {4},
   pages = {56-67},
   year = {2012},
   type = {Journal Article}
}

@article{Herkenhoffetal2016,
   author = {Herkenhoff, Kyle and Phillips, Gordon and Cohen-Cole, Ethan},
   title = {The Impact of Consumer Credit Access on Employment, Earnings, and Entrepreneurship},
   journal = {NBER Working Paper No. 22846},
   year = {2016},
   type = {Journal Article}
}

@article{HoffmanKahnLi2017,
   author = {Hoffman, Mitchell and Kahn, Lisa B and Li, Danielle},
   title = {Discretion in Hiring*},
   journal = {The Quarterly Journal of Economics},
   volume = {133},
   number = {2},
   pages = {765-800},
   year = {2017},
   type = {Journal Article}
}

@article{JaroschPilossoph2018,
   author = {Jarosch, Gregor and Pilossoph, Laura},
   title = {Statistical Discrimination and Duration Dependence in the Job Finding Rate},
   journal = {The Review of Economic Studies},
   year = {2018},
   type = {Journal Article}
}

@article{KahnLange2014,
   author = {Kahn, Lisa B. and Lange, Fabian},
   title = {Employer Learning, Productivity, and the Earnings Distribution: Evidence from Performance Measures},
   journal = {The Review of Economic Studies},
   volume = {81},
   number = {4},
   pages = {1575-1613},
   year = {2014},
   type = {Journal Article}
}

@article{Kroftetal2013,
   author = {Kroft, Kory and Lange, Fabian and Notowidigdo, Matthew J.},
   title = {Duration Dependence and Labor Market Conditions: Evidence from a Field Experiment*},
   journal = {The Quarterly Journal of Economics},
   volume = {128},
   number = {3},
   pages = {1123-1167},
   year = {2013},
   type = {Journal Article}
}

@article{Lange2007,
   author = {Lange, Fabian},
   title = {The Speed of Employer Learning},
   journal = {Journal of Labor Economics},
   volume = {25},
   number = {1},
   pages = {1-35},
   year = {2007},
   type = {Journal Article}
}

@article{LeibbrandtList2014,
   author = {Leibbrandt, Andreas and List, John A.},
   title = {Do Women Avoid Salary Negotiations? Evidence from a Large-Scale Natural Field Experiment},
   journal = {Management Science},
   volume = {61},
   number = {9},
   year = {2014},
   type = {Journal Article}
}

@article{Mas2017,
   author = {Mas, Alexandre},
   title = {Does Transparency Lead to Pay Compression?},
   journal = {Journal of Political Economy},
   volume = {125},
   number = {5},
   pages = {1683-1721},
   year = {2017},
   type = {Journal Article}
}

@article{McNichols2019,
	author = {McNichols, Drew},
	title = {Information and The Persistence of The Gender Wage Gap: Early Evidence from California's Salary History Ban},
	year = {2019},
	type = {Journal Article}
}

@article{HansenNichols2020, 
    author = {Hansen, Benjamin and McNichols, Drew}, 
    title = {Information and the Persistence of the Gender Wage Gap: Early Evidence from California's Salary History Ban}, 
    journal = {NBER Working Paper}, 
    year = {2020}, 
    type = {Journal Article},
}

@article{MeliSpindler2019,
	author = {Meli, Jeffrey and Spindler, James C.},
	title = {Salary History Bans and Gender Discrimination},
	journal = {Available at SSRN 3361431},
	year = {2019},
	type = {Journal Article}
}

@article{Oyeretal2011,
   author = {Oyer, Paul and Schaefer, Scott},
   title = {Personnel Economics: Hiring and Incentives},
   journal = {Handbook of Labor Economics, 2011},
   volume = {4},
   pages = {1769-1823},
   year = {2011},
   type = {Journal Article}
}

@article{Pallais2014,
   author = {Pallais, Amanda},
   title = {Inefficient Hiring in Entry-Level Labor Markets},
   journal = {American Economic Review},
   volume = {104},
   number = {11},
   pages = {3565-99},
   year = {2014},
   type = {Journal Article}
}

@article{PayScaleData,
	author = {PayScale},
	title = {Salary History Disclosure Data, Last Updated: August, 2019},
	year = {2019},
	type = {Journal Article}
}

@article{ShoagVeuger2016,
   author = {Shoag, Daniel and Veuger, Stan},
   title = {No Woman No Crime: Ban the Box, Employment, and Upskilling},
   journal = {HKS Working Paper},
   volume = {16-015},
   year = {2016},
   type = {Journal Article}
}

@article{Tinsleyetal2009,
   author = {Tinsley, Catherine H. and Cheldelin, Sandra I. and Schneider, Andrea Kupfer and Amanatullah, Emily T.},
   title = {Women at the Bargaining Table: Pitfalls and Prospects},
   journal = {Negotiation Journal},
   volume = {25},
   number = {2},
   pages = {233-248},
   year = {2009},
   type = {Journal Article}
}

@article{Veldman2017,
   author = {Veldman, Albertine},
   title = {Pay Transparency in the EU: A Legal Analysis of The Situation in the EU Member States, Iceland, Liechtenstein and Norway},
   journal = {European Commission},
   year = {2017},
   type = {Journal Article}
}

@article{Wozniak2015,
   author = {Wozniak, Abigail},
   title = {Discrimination and the Effects of Drug Testing on Black Employment},
   journal = {The Review of Economics and Statistics},
   volume = {97},
   number = {3},
   pages = {548-566},
   year = {2015},
   type = {Journal Article}
}

@article{Zhang2007,
   author = {Zhang, Ye},
   title = {Employer Learning Under Asymmetric Information: The Role of Job Mobility},
   journal = {Working Paper},
   year = {2007},
   type = {Journal Article}
}

@article{Archer1979,
    author = {Archer, R.L.}, 
    title = {Role of Personality and the Social Situation},
    journal = {Self-Disclosure: Origins, Patterns, and Implications of Openness in Interpersonal Relations},
    year = {1979},
    type = {Journal Article}
}

@article{Bernheim1994, 
    author = {Bernheim, Douglas B.}, 
    title = {A Theory of Conformity}, 
    journal = {Journal of Political Economy}, 
    volume = {102},
    number = {5},
    year = {1994},
    type = {Journal Article}
}

@article{Cranoretal1999,
    author = {Cranor, L.F. and Reagle, J. and Ackerman, M.S.},
    title = {Beyond Concern: Understanding Net Users’ Attitudes about Online Privacy},
    journal = {ATT Labs Research Technical Report},
    volume = {99.4.3},
    year = {1999},
    type = {Journal Article}
}

@article{Cozby1973,
    author = {Cozby, P.C.},
    title = {Self-Disclosure: A Literature Review},
    journal = {Psychological Bulletin},
    volume = {79},
    number = {2},
    pages = {73-91},
    year = {1973},
    type = {Journal Article}
}

@article{DAttoma2017,
    author = {D'Attoma, John and Volinturi, Clara and Steinmo, Sven},
    title = {Willing to share? Tax compliance and gender in Europe and America},
    journal = {Research and Politics}, 
    pages = {1-10},
    year = {2017},
    type = {Journal Article}
}

@article{Dullecketal2016,
    author = {Dulleck, Uwe and Fooken, Jonas and Newton, Cameron and Ristl, Andrea and Schaffner, Markus and Torgler, Benno},
    title = {Tax Compliance and Psychic Costs: Behavioral experimental evidence using a physiological marker},
    journal = {Journal of Public Economics},
    volume = {134},
    pages = {9-18},
    year = {2016},
    type = {Journal Article}
}

@article{EaglyChrvala1986,
    author = {Eagly, Alice H. and Chrvala, Carole},
    title = {Sex Differences in Conformity: Status and Gender Role Interpretations},
    journal = {Psychology of Women Quarterly},
    pages = {203-220},
    year = {1986},
    type = {Journal Article}
}

@article{ErardFeinstein1994,
    author = {Erard, Brian and Feinstein, Jonathan S.},
    title = {The role of moral sentiments and audit perceptions in tax compliance},
    journal = {Public Finance},
    volume = {49},
    pages = {70-89},
    year = {1994},
    type = {Journal Article}
}

@article{FletcherSpencer1984,
    author = {Fletcher, C. and Spencer, A.},
    title = {Sex of Candidate and Sex of Interviewer as Determinants of Self-Preservation  Orientation  in  Interviews:  An  Experimental  Study},
    journal = {International  Review  of Applied Psychology},
    volume = {33},
    pages = {305-313},
    year = {1984},
    type = {Journal Article}
}

@article{GhoshRoth2011,
    author = {Ghosh, Arpita and Roth, Aaron},
    title = {Selling  Privacy  at  Auction},
    journal = {Games and Economic Behavior},
    volume = {91},
    pages = {334-346},
    year = {2011},
    type = {Journal Article}
}

@article{GroschHolger2016,
    author = {Grosch, Kerstin and Holger, A. Rau},
    title = {Gender Differences in compliance: The role of social value orientation},
    journal = {GlobalFood Discussion Papers, University of Gottingen},
    volume = {88},
    year = {2016},
    type = {Journal Article}
}

@article{Hannetal2002,
    author = {Hann, Il-Horn and Hui, Kai-Lung and Lee, Tom and Png, I.n},
    title = {Online Information Privacy: Measuring the Cost Benefit Trade Off},
    journal = {ICIS 2002 Proceedings 1},
    year = {2002},
    type = {Journal Article}
}

@article{Hubermanetal2005,
    author = {Huberman, B.A. and Adar, E. and Fine, L.R.},
    title = {Valuating Privacy},
    journal = {IEEE Security and Privacy},
    volume = {3},
    number = {5},
    pages = {22-25},
    year = {2005},
    type = {Journal Article}
}

@article{Kleinbergetal2001,
    author = {Kleinberg, Jon and Papadimitriou, Christos H. and Raghavan, Prabhakar},
    title = {On the value of private  information},
    journal = {TARK01: Proceedings of the 8thConference  on  Theoretical  Aspects  of Rationality and Knowledge},
    year = {2001},
    type = {Journal Article}
}

@article{LigettRoth2012,
    author = {Ligett, Katrina and Roth, Aaron},
    title = {Take it or Leave it –Running a Survey when Privacy comes at a cost},
    journal = {Internet and Network Economics, WINE},
    pages = {378-391},
    year = {2012},
    type = {Journal Article}
}

@article{Nissimetal2014,
    author = {Nissim, Kobbi and Vadhan, Salil and Xiao, David},
    title = {Redrawing the boundaries on purchasing data from privacy-sensitive  individuals},
    journal = {ITCS14:Proceedings   of   the  5th Conference   on Innovations in Theoretical Computer Science},
    year = {2014},
    type = {Journal Article}
}

@article{Phelpsetal2000,
    author = {Phelps, J. and Nowak, G. and Ferell, E.},
    title = {Privacy Concerns and Consumer Willingness to Provide Personal Information},
    journal = {Journal of Public Policy and Marketing},
    volume = {19},
    number = {1},
    pages = {27-41},
    year = {2000},
    type = {Journal Article}
}

@article{RothSchoenbeck2012,
    author = {Roth, Aaron and Schoenbeck, Grant},
    title = {Conducting Truthful Surveys, Cheaply},
    journal = {EC’12: Proceedings of the 13th ACM Conference on Electronic Commerce},
    year = {2012},
    type = {Journal Article}
}

@article{Singeretal2001,
    author = {Singer, E. and Van Howeyk, J. and Tourangeau, R. and Steiger, D.M. and Montgomery, M. and Montgomery, R.},
    title = {Final  report  on  the  1999-2000  surveys of  privacy  attitudes.  Technical  report, Washington, DC, US Bureau of the Census, Planning, Research and Evaluation Division},
    year = {2001},
    type = {Journal Article}
}

@article{TomGranie2011,
    author = {Tom, Ariane and Granie Marie-Axelle},
    title = {Gender differences in pedestrian rule compliance and visual search in signalized and unsignalized crossroads},
    journal = {Accident Analysis and Prevention},
    volume = {43},
    pages = {1794-1801},
    year = {2011},
    type = {Journal Article}
}

@article{Waldoetal2007,
    author = {Waldo,  James  and  Lin,  Herbert  S.  and  Millett,  Lynette  I.},
    title = {Engaging  Privacy  and Information Technology in a Digital Age},
    year = {2007},
    type = {Journal Article}
}

@article{WathieuFreidman2007,
    author = {Wathieu, Luc and Freidman, Allan},
    title = {An Empirical Approach to Understanding Privacy Valuation},
    journal = {Harvard Business School Working Knowledge, Working Paper},
    year = {2007},
    type = {Journal Article}
}

@article{Brownetal2008,
   author = {Brown, Gordon D.A. and Gardner, Jonathan and Oswald, Andrew, J. and Qian, Jing},
   title = {Does Wage Rank Affect Employees' Well-Being?},
   journal = {Industrial Relations},
   volume = {47},
   number = {3},
   pages = {355-389},
   year = {2008},
   type = {Journal Article}
}

@article{Clarketal2009,
   author = {Clark, Andrew E. and Kristensen, Nicolai and Westergard-Nielsen, Niels},
   title = {Job Satisfaction and Co-Worker Wages: Status or Signal?},
   journal = {The Economic Journal},
   volume = {119},
   number = {536},
   pages = {430-447},
   year = {2009},
   type = {Journal Article}
}

@article{ClarkOswald1996,
   author = {Clark, Andrew E. and Oswald, Andrew J.},
   title = {Satisfaction and Comparison Income},
   journal = {Journal of Public Economics},
   volume = {61},
   number = {3},
   pages = {359-381},
   year = {1996},
   type = {Journal Article}
}

@article{GodechotSenik2015,
   author = {Godechot, Oliver and Senik, Claudia},
   title = {Wage Comparisons In and Out of Firm: Evidence from a Matched Employer-Employee French Database},
   journal = {Journal of Economic Behavior and Organization},
   volume = {117},
   pages = {395-410},
   year = {2015},
   type = {Journal Article}
}

@article{Luttmer2005,
   author = {Luttmer, Erzo F.P.},
   title = {Neighbors as Negatives: Relative Earnings and Well-Being},
   journal = {The Quarterly Journal of Economics},
   volume = {120},
   number = {3},
   pages = {963-1002},
   year = {2005},
   type = {Journal Article}
}

@article{Bennedsenetal2019,
   author = {Bennedsen, Morten and Simintzi, Elena and Tsoutsoura, Margarita and Wolfenzon, Daniel},
   title = {Do Firms Respond to Gender Pay Gap Transparency?},
   journal = {NBER Working Paper No. 25435},
   year = {2019},
   type = {Journal Article}
}

@Article{Blundell2020,
  author = {Blundell, Jack},
  title = {Wage responses to gender pay gap reporting requirements},
  journal = {Working Paper},
  year = {2020},
  type = {Journal Article},
}

@Article{Duchinietal2020,
  author = {Duchini, Emma and Simion, Stefania and Turrell, Arthur},
  title = {Pay Transparency and Cracks in the Glass Ceiling},
  journal = {Working Paper},
  year = {2020},
  type = {Journal Article},
}

@article{Gulyasetal2020,
    author = {Gulyas, Andreas and Seitz, Sebastian and Sinha, Sourav},
    title = {Does Pay Transparency Affect the Gender Wage Gap? Evidence From Austria},
    journal = {CRC TR 224 Discussion Paper Series}, 
    year = {2020}, 
    type = {Journal Article},
}

@article{Sinha2019,
    author = {Sinha, Sourav},
    title = {Salary History Ban: Gender Pay Gap and Spillover Effects}, 
    journal = {Available at SSRN},
    year = {2019},
    url = {https://ssrn.com/abstract=3458194},
    type = {Journal Article},
}

@article{Sranetal2020, 
    author = {Sran, Gurpal and Vetter, Felix and Walsh, Matthew}, 
    title = {Employer Responses to Pay History Enquiry Bans}, 
    journal = {Available at SSRN}, 
    year = {2020},
    url = {https://ssrn.com/abstract=3587736},
    type = {Journal Article},
}

@article{Bessenetal2020,
    author = {Bessen, James E. and Meng, Chen and Denk, Erich},
    title = {Perpetuating Inequality: What Salary History Bans Reveal About Wages}, 
    journal = {Available at SSRN}, 
    url = {https://ssrn.com/abstract=3628729}, 
    year = {2020}, 
    type = {Journal Article},
}

@article{Mask2021, 
    author = {Mask, Joshua}, 
    title = {Salary History Bans and Healing Scars from Past Regressions}, 
    journal = {Working Paper},
    year = {2021}, 
    type = {Journal Article}, 
}

@article{GoodmanBacon2021, 
    author = {Goodman-Bacon, Andrew}, 
    title = {Difference-in-Differences with Variation in Treatment Timing}, 
    journal = {Journal of Econometrics}, 
    year = {2021}, 
    type = {Journal Article},
}

@article{Chaisemartinetal2020, 
    author = {de Chaisemartin, Clement and D'Haultfoeuille, Xavier}, 
    title = {Two-Way Fixed Effects Estimators with Heterogeneous Treatment Effects}, 
    journal = {American Economic Review}, 
    volume = {110}, 
    number = {9}, 
    pages = {2964-96}, 
    year = {2020}, 
    type = {Journal Article},
}

@article{SunAbraham2020, 
    author = {Sun, Liyang and Abraham, Sarah}, 
    title = {Estimating dynamic treatment effects in event studies with heterogeneous treatment effects}, 
    journal = {Journal of Econometrics}, 
    year = {2020}, 
    type = {Journal Article},
}

@article{CallawaySantAnna2021, 
    author = {Callaway, Brantly and Sant'Anna, Pedro H.C.}, 
    title = {Difference-in-Differences with Multiple Time Periods}, 
    journal = {Journal of Econometrics}, 
    year = {2021}, 
    type = {Journal Article}, 
}

@article{CahucPostelVinayRobin2006, 
    author = {Cahuc, Pierre and Postel-Vinya, Fabian and Robin, Jean-Marc}, 
    title = {Wage Bargaining with On-The-Job Search: Theory and Evidence},
    journal = {Econometrica}, 
    volume = {74}, 
    number = {2}, 
    pages = {323-364}, 
    year = {2006}, 
    type = {Journal Article},
}

@article{PostelVinayRobin2002, 
    author = {Postel-Vinay, Fabian and Robin, Jean-Marc}, 
    title = {Equilibrium Wage Dispersion with Worker and Employer Heterogeneity}, 
    journal = {Econometrica}, 
    volume = {70}, 
    number = {6}, 
    pages = {2295-2350}, 
    year = {2002},
    type = {Journal Article},
}

@article{Baggeretal2014, 
    author = {Bagger, Jesper and Fontaine, Francois and Postel-Vinay, Fabian and Robin, Jean-Marc}, 
    title = {Tenure, Experience, Human Capital, and Wages: A Tractable Equilibrium Search Model of Wage Dynamics}, 
    journal = {American Economic Review}, 
    volume = {104}, 
    number = {6}, 
    pages = {1551-1596}, 
    year = {2014}, 
    type = {Journal Article},
}

@article{CPSData, 
    author={Flood, Sarah and King, Miriam and Rodgers, Renae and Ruggles, Steven and Warren, Robert J. and Westberry, Michael}, 
    title={Integrated Public Use Microdata Series, Current Population Survey}, 
    volume={9.0}, 
    year={2021}, 
    url={https://doi.org/10.18128/D030.V9.0},
}



@Comment{jabref-meta: databaseType:bibtex;}


